Characterisation of the VELO High Voltage System

The high voltage system supplies the bias voltage to the 88 silicon sensors which comprise the LHCb Vertex Locator (VELO). This note describes the results of the tests which have been performed on the hardware of the high voltage system of the VELO. Each individual test detailed in this note corresponds to a specific requirement of the system. These requirements arise primarily from ensuring the safety of the silicon sensors and the quality of the data taken from the VELO modules. The tests performed are in four categories: normal operation of the high voltage system; verification of its stability under operation; discussion of its behaviour in failure modes; and details of operation at low voltage. Noteworthy issues, identified through the tests, include the behaviour of the high voltage modules at voltages below 9V, the current limit that can be applied during ramping of the voltage, and the speed with which the voltage is cut during failures of the system. The results of these tests provide high confidence that the high voltage system can be safely used and demonstrate that low noise is produced by the power supplies.

==> control_and_data/control_intro.tex <==
\subsection{Control and Data Acquisition}

The data acquisition setup (DAQ) used in the burn-in lab was able to fully 
operate the electronics of the module and acquire data from both sides of the 
module simultaneously inside 
the vacuum chamber. This DAQ electronics was quite similar to the ones that will be used in the final experiment. Figure 
\ref{DAQ_scheme} illustrates how the DAQ used in the burn-in was set up.

\begin{figure}[t!!!!!!!!!]
\begin{center}
\epsfig{file=daq_diagram.eps,width=1.0\textwidth}
\caption[]{Diagram of the DAQ system in the burn-in. The readout supervisor 
sends TFC signals to the Beetle front-end chips in order to configure them. The
data acquired is received and digitised by the Tell1 boards and then stored in 
binary files in a Linux machine.}
\label{DAQ_scheme}
\end{center}
\end{figure}

The Odin readout supervisor was responsible for the control of the modules readout 
\cite{READSUPER}.
It was done by sending TFC signals to the control board \cite{CTRLBOARD} and Tell1 mother boards \cite{TELL1}.
The control board sent these signals to the Beetle chips in the modules via 
the repeater boards in order to configure and operate them. The data acquired 
was sent back to the Tell1 boards passing through the repeater boards. The Tell1
boards digitise the data and it was finally acquired by a Linux machine by means
of Gigabit Ethernet cards. The Linux machine saved the data in a binary file 
for further analysis.

\subsubsection{Data Readout}

The DAQ hardware consists of two Tell1 mother boards, two repeater boards, one 
control board and one Odin readout supervisor. The Tell1 mother boards, control board and readout supervisor were located in a single crate. The repeater boards were placed close to the chamber lid. Figure \ref{DAQ_pic} shows the 
setup. The Tell1 boards are connected to the repeater boards via 8 data cables each 5 m long. Two control cables connect the repeater boards to the 
control board and each cable is 20 m long. To connect the repeater boards to the hybrid 
four pcb patch cards are plugged on the lid of the vacuum tank and sealed on 
the outside and inside of the chamber. Between the pcb patch cards and repeater boards there 
are 8 flat 50 pin cables 10 cm long with strain relief connectors. Finally the 
modules kapton cables are connected directly to the patch cards. 

\begin{figure}
\begin{center}
\epsfig{file=daq_burnin.eps,width=1.0\textwidth}
\caption[]{The DAQ setup in the burn-in system.}
\label{DAQ_pic}
\end{center}
\end{figure}

In the LHCb experiment, the timing and fast control (TFC) distributes the
information that has to arrive synchronously at different points of the 
experiment \cite{TFC}. The readout supervisor is the component of the LHCb TFC 
that is
responsible for the distribution to the front-end electronics of the timing, 
trigger and control commands necessary for the synchronous readout. It also
acts as trigger rate controller avoiding buffer overflows using the status
of the different components of the system.

The control board receives the timing signals and fast commands from the 
Readout Supervisor and distributes them to the Level 0 electronics. Each
control board can support up to 6 VELO modules. The configuration data 
on the control board are translated and distributed to the configurable 
components via I$\rm ^2$C by the Specs Slave on the board \cite{SPECS}. Specs is a  
10 Mbit/s serial link based on master multi-slave paradigm designed for the 
configuration of remote electronics elements. It is used to read the 
configuration of the electronics located on the detector. It allows fast, 
efficient and error safe communication between electronic elements. On the 
experiment the monitored voltages are digitised on the control board and sent 
to the experiment control system (ECS).

The repeater board acts as a signal amplifier of the TFC and configuration
commands from the control board as for the data signals read from the 
detector front-end. The control commands to the repeater boards are sent only by
the control board. It also contains drivers and multiplexers for the 
monitoring signals. The monitoring signals are of two types: temperature 
monitoring signals and voltage monitoring signals. In the LHCb experiment
the monitoring signals will be routed either to the so-called temperature 
board or to the control board. The temperature monitoring and interlock of the 
modules and repeater board will be made by the temperature board. However, in 
the burn-in system the temperature monitoring is performed using a Keithley 
and the temperature interlock done by a custom made unit (see Sections 
\ref{monitor} and \ref{inter_sys}).

A FPGA based acquisition board was developed for the LHCb experiment. The 
so-called Tell1 board is used on all sub-detectors in the experiment. Its 
design and functionality is constrained by the maximum L0 output event rate of 
1.1MHz. Its makes the interface between the sub-detectors front-end electronics
and the DAQ network. It can also perform basic data preprocessing. 

The Tell1 works as a receiver card of the front-end electronics signals. On the
VELO such data is delivered via analogue electronic signals which are digitised 
on the analogue receiver side. The Tell1 board can accept electrical or optical 
signal input cards depending on the sub-detector it will read out. To perform 
the main preprocessing of the 1.1MHz L0 accepted data the Tell1 boards have 4 
PP-FPGAs (Pre Processor FPGAs). Some of the data processing steps that the 
Tell1 can perform on the data from the Beetle chips on the VELO modules are the
pedestal subtraction, data reordering, clusterization, Finite Impulse Response filter correction (FIR) and 
common mode correction. In the burn-in lab only the digitised raw data was 
saved and the processing was performed afterwards. The SyncLink-FPGA collects 
the data from the PP-FPGAs and assembles the data fragments. Then various 
events are put together into multiple events packages (MEP) before its 
transmission to the DAQ network. The SyncLink-FPGA also distributes the 
synchronisation signals to the PP-FPGAs. The data is then delivered to the DAQ 
network via a Gigabit Ethernet card (GBE).

A Linux machine equipped with a Gigabit Ethernet card is used to acquire the 
data from the Tell1 boards and write it in binary files. The files are analysed
with the Gaudi based Vetra package \cite{VETRA}. It is used to perform processing stages 
such as the pedestal evaluation and the common mode suppression of the data, 
saving the results in ROOT files. The final analysis to estimate noise, signal 
to noise and number of bad strips on the silicon sensors is done using ROOT 
scripts. 

\subsubsection{Software}

The software panels to control the hardware in LHCb are made within the PVSS
framework \cite{PVSS}. It is an application that allows the development of supervisory 
control and data acquisition systems (SCADA). It has been used in the LHC 
experiments and is widely used on industrial applications to control 
distributed system from a master location. In LHCb it is used to access the
DAQ hardware slow controls such that it can be initialised, configured and 
operated. It can connect to the hardware devices, acquire data and monitor 
their behaviour.

The communication between the PVSS applications and the CCPCs in the burn-in
lab are done with the client-server paradigm. These applications allows the user
to initialise and operate all the boards in order to run the data acquisition
system. Hence, the VELO modules operation is also controlled by the system user
via the PVSS applications. 

The credit card PCs (CCPC) runs a server while the PVSS applications run 
clients. By means of the client the application demands the server to execute 
some task it can perform according to the functionality it has implemented. To 
perform the FPGAs programming directly a generic server is available on the 
CCPCs. It is referred to as the DIM server since it was implemented with the
Distributed Information Management package \cite{DIM}.

To operate the whole DAQ system a set of servers has to be initialised. To 
set up the Odin one has to start its server and depending on the type of task 
it will perform different recipes are loaded. The Odin server runs 
automatically. In order to operate the control board correctly the Specs server have to be 
running properly. In the final experiment the Tell1 boards will also run 
servers but up to now it has been operated by direct Linux commands in the 
burn-in lab.




==> failure_modes/currentfluctuation.tex <==
\subsection{Current Reading Fluctuation}

The tests that have been peformed to all channels of the High Voltage System showed a current reading fluctuation. The peak-to-peak
amplitude of the fluctuation is up to 1$\mu$A. This behavior has been seen without anything connected at the output of the High Voltage Modules, also 
by putting a resistance of 100M$\Omega$ at 100V.
A voltage of 100V applied to this resistance of 100M$\Omega$ with 10$\%$ gives a displayed current between 1$\mu$A and 2$\mu$A. 
This is a proof that the fluctuation observed is only a current display problem.
The voltage was set and measured using the Iseg stand alone control software IsegHVControl version 1.57. 
In addition, a comparison has been made by using PVSS, by mean the Iseg OPC server 5.0006 has been used. Both software showed the same measured current behavior.
This behaviour has been reported to Iseg. 


\subsection{Instantaneous ramp down}

The stress test that were performed to the Iseg Modules has revealed a bug in the actual firware 2.04 of the High Voltage Modules. 
An instaneous ramp down occurs to all channels of the same board which ramp down if at least one channel that ramps down receives a command to switch on.
The same problem have been seen either by using the Iseg stand alone control software IsegHVControl version 1.57 or PVSS through the  Iseg OPC server 5.00.0006.
The problem has been reported and was reproduced by Iseg. Iseg has released a new version of the High Voltage Module 
firmware, also the version 1.58 of the IsegHVControl.
A futur upgrade to this new firmare version is considered in longer timescale due to the bad experience with upgrading the firmware of one spare High Voltage Module.
This upgrade led to crash one of the two boards of the High Voltage Module.  




==> kill_enable/kill_enable.tex <==



==> performance/franciole_performance_intro.tex <==
\section{Conclusion}\label{conclusion}


A facility has been developed and commisioned to perform the reception,
visual inspection and burn-in of the VELO modules. The reception and visual 
inspection checks aim to verify the physical integrity of the modules on their
 arrival and after the burn-in tests. The burn-in setup can be used to perform a long term evaluation of the modules in environmental conditions similar to those in the real LHCb experiment. The modules are thermally stressed in order to uncover any latent weakness intrinsic to the components of the module or introduced during the assembly phase.  

Procedures and suitable mechanics have been developed for the safe handling of the modules during reception and visual inspection. A transfer jig and an aluminium frame with a base compatible with the module attachment points have been made. When the module is mounted on this frame transparent plastic plates are used to protect the module. The frame fits safely under the microscope to allow visualisation of the different elements of the module.

The burn-in setup is composed of vacuum, cooling, DAQ, interlock and 
monitoring systems. These components were developed to allow the modules
to be operated under the required environmental conditions. Satisfactory performance of these components has been achieved such that the VELO modules can be
operated according to the requirements specified for the burn-in tests.

The vacuum system consists of a set of vacuum pumps and a vacuum chamber. 
The obtained values of pressure obtained in the burn-in setup are adequate
to test the module in a environment similar to the LHCb experiment. The system 
achieved pressure levels of the order of 5-10$\times$10$^{-5}$ mbar within
a period of 20 to 40 minutes. Running overnight values of about 0.5-1 
$\times$10$^{-5}$ mbar were reached. 

The cooling system was designed to provide appropriate heat transfer from
the module to the coolant liquid used. The critical part of the design of 
this system is the cooling block. A set of mechanical constraints lead the
cooling block to be a two piece cooper pipe connected by a U tube. This
connection allows the cooling pipe to expand and contract  according to
the temperature changes without applying mechanical stress on the module.
The final cooling block is able to cool down a mounted module from 30.0
$\rm ^{o}$C to -20.0 $\rm ^{o}$C in about 20 minutes. A similar period of time 
is taken to bring the module temperature up again.  

The burn-in DAQ system has been used to acquire data from the modules. It 
can read out both sides of the module simultaneously using two Tell1 boards. 
To set up the correct chip configuration a control board is used. Repeater 
boards are necessary to shape and amplify the signals read out from the Beetle
chips and serve the modules with voltages and currents. The acquired data is 
digitised by the Tell1 boards and them saved onto disk using Gigabit Ethernet
cards to transfer the data to the Linux machine available in the lab. 
Afterwards the data is stored and can be analysed with the data analysis 
software that has been developed.

A set of possible failure modes were identified in the burn-in system and to 
protect the modules against any possible malfunction an interlock system was 
developed. It consists of two units which are used to monitor the temperature 
of the modules inside the tank and the pressure. If a failure in the 
cooling system causes overheating the temperature hardware interlock will shut
down the low voltage and high voltage supply to the module. If the vacuum system stops pumping down, raising the pressure, then the pressure hardware interlock units will also turn off the module. 

The Glasgow burn-in facility has been commisioned and achieved the requirements necessary to allow the testing of the VELO modules, suitably replicating the LHCb environment. The vacuum system provides the low pressure needed within a reasonable time scale. The cooling system is able to thermal cycle the cooling block and control the hybrid temperature. A DAQ system to readout both sides of the 
module simultaneously has been operated. The safety of the modules during the tests is ensured by a hardware interlock system monitoring both pressure and 
temperature of the module.







==> performance/performance_intro.tex <==
\section{Conclusion}\label{conclusion}

A full setup has been developed to perform the reception,
visual inspection and burn-in of every VELO module. The reception and visual inspection aim to verify the physical integrity of the modules at arrival time 
and after the burn-in tests. The burn-in setup allows to test the modules
in environmental conditions similar to the real LHCb experiment. It also
thermally stresses the modules in order to uncover any weakness 
introduced on the components of the module or during the assembly phase.  

To perform the handling of the modules during reception and visual inspection 
a full setup was used. A transfer jig and an aluminium frame with compatible
basis to the module attachment have been made. When the module is mounted on this
frame clean plastic plates are used to protect the module. The frame is such
that it fits on microscope being easy and safe to visualise the different 
parts of the module. Appropriate procedures were developed to handle the module
in the most safe manner.

The burn-in setup is composed of vacuum, cooling, DAQ, interlocks and 
monitoring systems. These components were developed to allow the modules
to be operated under the required conditions. Satisfactory performance of
these components has been achieved such that the VELO modules can be
operated according to the requirements.

The vacuum system consists of a set of vacuum pumps and vacuum chamber. 
The obtained values of pressure obtained in the burn-in setup are adequate
to test the module in a environment similar to the LHCb experiment. It 
achieves pressure levels of the order of 5-10$\times$10$^{-5}$ Torr within
a period of 20 to 40 minutes. Running overnight values of about 5 
$\times$10$^{-6}$ Torr were reach. 

The cooling system was designed to provide appropriate heat transfer from
the module to the coolant liquid used. The critical part of the design of 
this system is the cooling block. A set of mechanical constraints lead the
cooling block to be a two piece cooper pipe connected by a U tube. This
connection allows the cooling pipe to expands and contracts according to
its temperature changes without applying any mechanical stress on the module.
The final cooling block is able to cool down a mounted module from 30.0
$\rm ^{o}$C to -20.0 $\rm ^{o}$C in about 20 minutes. The same period of time 
is taken to bring the module temperature up again.  

The burn-in DAQ system has been used to acquire the data from the modules. It 
can read out both sides of the module simultaneously using two Tell1 boards. To 
set up the correct chip configuration a control board is used. Repeater 
boards are necessary to shape and amplify the signals read out from the Beetle
chips and serve the modules with voltages and currents. The acquired data is 
digitised by the Tell1 boards and them dumped into disk using Gigabit Ethernet
cards to transfer the data to the Linux machine available in the lab. 
Afterwords the data is stored and can be analysed with the data analysis 
software available.

A set of possible failure modes were identified in the burn-in system and to protect
the modules against any possible malfunction of it a interlock system was 
developed. It consists of two units to monitor used to monitor the temperature 
of the modules inside the tank and the its pressure. If a failure on the 
cooling system causes overheating the temperature hardware interlock will shut
down the low voltage and high voltage supply to the module. It will prevent the
module to continue heating. If the vacuum system stops to pump down raising the
pressure the pressure hardware interlock units will also turn off the module. 

The Glasgow burn-in facility has achieved the requirements necessary to allow 
the testing of the VELO modules replicating the LHCb environment. The vacuum
system provided the low pressure needed within an reasonable time scale. The 
cooling system was able to thermal cycle the cooling block and 
control the hybrid temperature. An DAQ system to readout both sides of the 
module simultaneously was available. The modules safety during the tests was 
ensured by an hardware interlock system monitoring both pressure and 
temperature of the module.

%Both units have been tested in simulated situations without a module mounted
%on the chamber. The temperature interlock have been tested with a 10k$\Omega$ 
%NTC connected directly to the input. Using a hot air gun the NTC was heated and
%the unit relays opened their electrical contacts as expected. The pressure 
%interlock was verified using the burn-in vacuum system but also without a
%module mounted. The pumps were turned off and the pressure hardware interlock
%relays opened their electrical contacts as expected. 


%The interlock system was
%never triggered during operation of the modules in the burn-in system since
%no system failures have happened during this period.


